Faster Sampling via Stochastic Gradient Proximal Sampler

Stochastic gradients have been widely integrated into Langevin-based methods to improve their scalability and efficiency in solving large-scale sampling problems. However, the proximal sampler, which exhibits much faster convergence than Langevin-based algorithms in the deterministic setting Lee et al. (2021), has yet to be explored in its stochastic variants. In this paper, we study the Stochastic Proximal Samplers (SPS) for sampling from non-log-concave distributions. We first establish a general framework for implementing stochastic proximal samplers and establish the convergence theory accordingly. We show that the convergence to the target distribution can be guaranteed as long as the second moment of the algorithm trajectory is bounded and restricted Gaussian oracles can be well approximated. We then provide two implementable variants based on Stochastic gradient Langevin dynamics (SGLD) and Metropolis-adjusted Langevin algorithm (MALA), giving rise to SPS-SGLD and SPS-MALA. We further show that SPS-SGLD and SPS-MALA can achieve $\epsilon$-sampling error in total variation (TV) distance within $\tilde{\mathcal{O}}(d\epsilon^{-2})$ and $\tilde{\mathcal{O}}(d^{1/2}\epsilon^{-2})$ gradient complexities, which outperform the best-known result by at least an $\tilde{\mathcal{O}}(d^{1/3})$ factor. This enhancement in performance is corroborated by our empirical studies on synthetic data with various dimensions, demonstrating the efficiency of our proposed algorithm.

==> 0_config/init_load_icml_ver.tex <==
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{lipsum}         % Can be removed after putting your text content
\usepackage{natbib}
\usepackage{doi}
\usepackage{amssymb}
\usepackage{xcolor}         % colors
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{xspace}
\usepackage{lmodern}
\usepackage{diagbox}

\usepackage{enumitem}


% For paper revision:

\newcommand{\xh}[1]{\textcolor[HTML]{66CCFF}{#1}}
\def \dz {\textcolor{red}}

==> 0_config/math_commands_icml_ver.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\RR}{{\mathbb R}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


\newcommand{\issue}[1]{{\textcolor{purple}{#1} }}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~(\ref{#1})}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rvzeta{{\mathbf{\zeta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\cR{{\mathcal{R}}}
\def\EE{{\mathbb{E}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vrho{{\bm{\rho}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vmu{{\bm{\mu}}}
\def\vsigma{{\bm{\sigma}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}




% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

%

\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny{#1}};}}
% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}[2]{\mathrm{KL}\left(#1 \big\| #2\right)}
\newcommand{\FI}[2]{\mathrm{FI}\left(#1 \| #2\right)}
\newcommand{\TVD}[2]{\mathrm{TV}\left(#1, #2\right)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\newcommand{\der}{\mathrm{d}}
\newcommand{\fder}{\mathrm{D}}
\newcommand{\rgrad}{\mathrm{grad}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% Table settings

\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3\arrayrulewidth}

\newcommand{\tabitem}{~~\llap{\textbullet}~~}

% Lemma settings


%Specific Notations for Sampling along the Reverse Process with Recursive Score Estimation

\newcommand{\rbkwx}{\rvx^{\gets}}
\newcommand{\bkwx}{\vx^{\gets}}
\newcommand{\rbkwv}{\rvv^{\gets}}
\newcommand{\bkwv}{\vv^{\gets}}
\newcommand{\bkwp}{p^{\gets}}
\newcommand{\bkw}[1]{#1^{\gets}}

==> 0_contents/030framework_icml_ver.tex <==
\section{Proposed Framework}
\label{sec:framw}
This section will first introduce the notations commonly used in the following sections.
Then, we will specify the assumptions that the target distribution $p_*$ is required in our algorithms and analysis.
After that, the proposed framework and some fundamental properties, such as the error propagation control when sampling from an inexact conditional density $p_*^\prime(\vx|\vy)$, will be shown.


\begin{table*}[t]
    \scriptsize
    \centering
    \begin{tabular}{ccccc}
    \toprule
     Results & Algorithm & Assumptions & Metric & Complexity \\
     \midrule
     \citet{raginsky2017non} & SGLD & Dissipative, Component Smooth & $\mathcal{W}_2$ & $\tilde{\mathcal{O}}(\mathrm{poly}(d) \epsilon^{-4})$\\
     \midrule
     \citet{zou2021faster} & SGLD & Dissipative, Warm Start, Component Smooth & $\mathrm{TV}$ & $\tilde{\mathcal{O}}(d^4 \epsilon^{-2})$\\
     \midrule
     \citet{das2023utilising} & AB-SGLD & LSI, Finite-Sum, Smooth  &  $\mathrm{TV}$ & $\tilde{\mathcal{\mathcal{O}}}(d^{3/2} \epsilon^{-2})$\\
     \midrule
     \citet{das2023utilising} & CC-SGLD & LSI, $6^{\mathrm{th}}$ moment, Smooth &  $\mathrm{TV}$ & $\tilde{\mathcal{O}}(d^{4/3} \epsilon^{-2})$\\
     \midrule
     Theorem~\ref{thm:conv_gra_comp_innerSGLD_informal} & SPS-SGLD & LSI, Finite-Sum, Component Smooth & $\mathrm{TV}$ & \textcolor{red}{$\tilde{\mathcal{O}}(d\epsilon^{-2})$}\\
     \midrule
     Theorem~\ref{thm:conv_gra_comp_innerMALA_informal} & SPS-MALA & LSI, Finite-Sum, Component Smooth & $\mathrm{TV}$ & \textcolor{red}{$\tilde{\mathcal{O}}(d^{1/2}\epsilon^{-2})$}\\
     \bottomrule 
    \end{tabular}
    \caption{Comparison with prior works for SGLD. $d$ and $\epsilon$ mean the dimension and error tolerance. Note that we do not list the assumptions about the stochastic gradient since they vary greatly in different references, which will be discussed in our detailed theorems.
    The results of our theorem based on~\ref{con_ass:var_bound} and $\sigma^2 = \Theta(1)$. 
    Compared with the state-of-the-art result, the sampling methods with the stochastic proximal sampler have a better convergence rate with an $\tilde{\mathcal{O}}(d^{1/3})$ factor at least.} 
    \label{tab:comp_old}
    % \vspace{-14pt}
\end{table*}


\subsection{Notations and Assumptions}
\label{sec:no_and_ass}
We suppose the target distribution, i.e., $p_*\propto \exp(-f)$ with a finite sum negative log-density, which means
\begin{equation}
    \label{def:total_loss}
    f(\vx)\coloneqq \frac{1}{n}\sum_{i=1}^n f_i(\vx)\quad \mathrm{where}\quad \forall i,  f_i\colon \R^d\rightarrow \R.
\end{equation}
We use letters, e.g., $\vx$ and $\rvx$, to denote vectors and random vectors in $\R^d$ except for letters $\vb$ and $\rvb$, which denote sets and randomized sets.
The function $f_{\vb}$ denotes the energy function deduced by mini-batch $\vb$, i.e.,
\begin{equation}
    \label{def:minibatch_loss}
    f_{\vb}(\vx)\coloneqq \frac{1}{|\vb|}\sum_{i\in \vb}f_i(\vx)\quad \mathrm{where}\quad \vb\subseteq \{1,2,\ldots\, n\},
\end{equation}
and $\grad f_{\vb}$ is the corresponding mini-batch gradient. 
The notation $|\cdot|$ denotes the $L_1$ norm or the number of elements when the inner notation is a vector or a set, respectively.
The Euclidean norm (vector) and its induced norm (matrix) are denoted by $\|\cdot \|$.
For distributions $p$ and $q$, we use $\TVD{p}{q}$ and $\KL{p}{q}$ to denote their TV distance and KL divergence, respectively.

% the TV distance and KL divergence are denoted by
% \begin{align}
% \TVD{p}{q}\coloneqq \frac{1}{2}\int |p(\vx)-q(\vx)|\der \vx,\tag{TVD}\\
% \KL{p}{q}\coloneqq \int p(\vx)\log \frac{p(\vx)}{q(\vx)}\der\vx. \tag{KL}
% \end{align}
Then, we show the assumptions required for $p_*$:
\begin{enumerate}[label=\textbf{[A{\arabic*}]},nosep]
    \item  
    \label{con_ass:lips_loss}(Component Smooth) For any $i\in\{1,2,\ldots, n\}$, the gradient of $f_i$ is $L$-smooth, which means
    \begin{equation*}
        \left\|\grad f_i(\vx) - \grad f_i(\vy)\right\| \le L\left\|\vx-\vy\right\|.
    \end{equation*}
    %\item \label{con_ass:second_moment} The target distribution has a bounded second moment, i.e., $M\coloneqq \mathbb{E}_{p_*}[\left\|\cdot\right\|^{2}]<\infty$.
    \item \label{con_ass:lsi}(Log-Sobolev Inequality) The target distribution $p_*$ satisfies the following inequality 
    \begin{equation*}
        \begin{aligned}
            &\E_{p_*}\left[g^2\log g^2\right]-\E_{p_*}[g^2]\log \E_{p_*}[g^2]
            \le \frac{2}{\alpha_*} \E_{p_*}\left\|\grad g\right\|^2
        \end{aligned}
    \end{equation*}
    with a constant $\alpha_*$ for all smooth function $g\colon \R^d\rightarrow \R$ satisfying $\E_{p_*}[g^2]<\infty$.
    \item \label{con_ass:var_bound}(Bounded Variance) For any $\vx\in\R^d$, the variance of stochastic gradients is bounded, i.e., 
    \begin{equation*}
        \frac{1}{n}\sum_{i=1}^n \left\|\grad f_i(\vx)-\grad f(\vx)\right\|^2\le \sigma^2.
    \end{equation*}
\end{enumerate}
The component smoothness of the finite sum loss, i.e.,~\ref{con_ass:lips_loss}, is also required in~\citet{raginsky2017non,zou2021faster}.
%~\ref{con_ass:second_moment} is a common assumption that requires the target distribution to belong to Wasserstein $2$ space shown in~\cite{vempala2019rapid}.
\ref{con_ass:lsi} is a kind of isoperimetric condition~\cite{vempala2019rapid} which is strictly weaker than the strongly log-concave assumption and even the dissipative assumption~\cite{raginsky2017non}.
Besides, it implies the target distribution $p_*$ to have a finite second moment $M$ satisfying $M=\mathcal{O}(d)$, which is demonstrated in Appendix~\ref{sec:not_ass_0x}.
~\ref{con_ass:var_bound} recovers the standard
uniformly bounded variance assumption, i.e., $\sigma=\Theta(1)$, following from~\citet{nemirovski2009robust,ghadimi2012optimal,ghadimi2013stochastic}, and sampling references sometimes allow $\sigma^2 = \Theta(d)$, e.g., ~\citet{raginsky2017non, dalalyan2019user, das2023utilising}.
Both of these cases will be considered in our analysis.

\begin{algorithm}[t]
    \caption{Stochastic Proximal Sampler}
    \label{alg:sps}
    \begin{algorithmic}[1]
            \STATE {\bfseries Input:} The negative log density $f$ of the target distribution, the initial particle $\rvx_0$ drawn from $p_0$;
            \FOR{$k=0$ to $K-1$}
                \STATE Sample $\hat{\rvx}_{k+1/2}$ from $\hat{p}_{k+1/2|k}(\cdot|\rvx_k)$;
                \STATE Draw the mini-batch $\rvb_k$ from $\{1,2,\ldots, n\}$;
                \STATE Sample $\hat{\rvx}_{k+1}$ from  $\hat{p}_{k+1|k+1/2,b}(\cdot|\hat{\rvx}_{k+1/2},\rvb_k)$;
            \ENDFOR
            \STATE {\bfseries Return:} $\hat{\rvx}_{K}$.
    \end{algorithmic}
\end{algorithm}



\subsection{Stochastic Proximal Sampler}
The stochastic proximal sampler (SPS) framework is shown in Alg.~\ref{alg:sps}.
With the common notations introduced in Section~\ref{sec:no_and_ass}, we will explain $\hat{p}_{k+1/2|k}(\cdot|\rvx_k)$ and $\hat{p}_{k+1|k+1/2,b}(\cdot|\rvx_{k+1/2},\rvb_k)$, that are similar to standard proximal samplers.
Considering a joint target distribution 
\begin{equation}
    \label{def:joint_target_rand}
    p_*(\vx,\vy) \propto \exp\bigg(-f_{\rvb}(\vx)-\frac{\left\|\vx-\vy\right\|^2}{2\eta}\bigg)
\end{equation}
%\dz{definition for $\eta_k$ is missing}
that is defined by the randomized mini-batch $\rvb$ and the outer loop step size $\eta$, then Alg.~\ref{alg:sps} samples from $p_*^\prime(\vy|\vx)$ and $p_*^\prime(\vx|\vy)$ alternatively.
Specifically, at iteration $k$, suppose $\vx=\vx_k$, $\vy=\vx_{k+1/2}$ and $\eta=\eta_k$, the conditional probability density $p_*^\prime(\vx_{k+1/2}|\vx_k)$ is equivalent to 
\begin{equation}
    \small
    \label{def:transition_kernel_stage1}
    p_{k+\frac{1}{2}|k}(\vx^\prime|\vx) \propto \exp\left(-\frac{\left\|\vx^\prime - \vx\right\|^2}{2\eta_k}\right),
\end{equation}
which can be exactly implemented by Line 3 of Alg.~\ref{alg:sps} due to its Gaussianity.
Besides, suppose $\vx=\vx_{k+1}$ and $\vy=\vx_{k+1/2}$, the transition kernel $p_*^\prime(\vx_{k+1}|\vx_{k+1/2})$ can be reformulated as
\begin{equation}
    \small
    \label{def:transition_kernel_stage2}
    \begin{aligned}
        p_{k+1|k+\frac{1}{2},b}(\vx^\prime|\vx, \vb) \propto \exp\left(-f_\vb(\vx^\prime)-\frac{\left\|\vx^\prime - \vx\right\|^2}{2\eta_k}\right),
    \end{aligned}
\end{equation}
which is desired to be implemented with Line 5 of Alg.~\ref{alg:sps}.
Rather than exactly sampling from a target distribution, e.g., $p_{k+1|k+\frac{1}{2},b}(\vx^\prime|\vx,\vb)$, most samplers can only generate approximate samples that are close to the target ones in real practice.
Therefore, we consider a Markov process $\{\hat{\rvx}_k\}$ whose underlying distribution is defined as $\hat{p}_k$.
Given the same initialization $\hat{p}_0 = p_0$, we denote the two empirical transition kernels as $\hat{p}_{k+\frac{1}{2}|k} \coloneqq p_{k+\frac{1}{2}|k}$ and $\hat{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)$ that satisfies
\begin{equation}
    \label{def:transition_kernel_norgo}
    \begin{aligned}
        \KL{\hat{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)}{{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)} \le \delta_k.
    \end{aligned}
\end{equation}
Here we assume that the conditional distribution of $\hat{\rvx}_{k+1}$ given $\hat{\rvx}_{k+1/2}$ is close to the ideal conditional distribution  $p_{k+1|k+1/2,b}(\vx^\prime|\vx, \vb)$ with up to $\delta_k$ approximation error in KL divergence. 
In fact, as the distribution  $p_{k+1|k+1/2,b}(\vx^\prime|\vx, \vb)$ is strongly log-concave when $\eta_k$ is properly chosen, the condition Eq.~\ref{def:transition_kernel_norgo} can be achieved by applying standard numerical samplers such as SGLD and MALA with provable guarantees (detailed implementations will be discussed in the next section). 

Then, the following theorem characterizes the error propagation across multiple steps and provides general results on the sampling error achieved by Alg.~\ref{alg:sps}.




% To describe the error propagation with the iteration growth, we have the following two results corresponding to the cases when $\delta_k=0$ and $\delta_k\not=0$.
% \begin{theorem}
%     \label{thm:tv_bound_rgo}
%     Suppose Assumption~\ref{con_ass:lips_loss}-\ref{con_ass:var_bound} hold, and Alg.~\ref{alg:sps} satisfy:
%     \begin{itemize}
%         \item The step sizes have $\eta_i\le 1/(2L)$ for all $i\in\{0,1,\ldots, K-1\}$.
%         \item The initial particle $\hat{\rvx}_0$ is drawn from the standard Gaussian distribution on $\R^d$.
%         \item The transition kernel at Line 5 of Alg.~\ref{alg:sps}, i.e., $\hat{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)$, satisfies Eq~\ref{def:transition_kernel_norgo} and $\delta_k=0$.
%     \end{itemize}
%     Then, we have
%     \begin{small}
%     \begin{equation*}
%         \TVD{\hat{p}_{K}}{p_*} \le \sigma \sqrt{\sum_{i=0}^{K-1} \frac{\eta_i}{2|\rvb_i|}} + \sqrt{\frac{(1+L^2)d}{4\alpha_*}} \cdot \prod_{i=0}^{K-1} \left(1+\alpha_* \eta_i\right)^{-1}. 
%     \end{equation*}
%     \end{small}
% \end{theorem}
% When the sample size $|\rvb_i|$, is large enough, e.g., $|\rvb_i|=\tilde{O}(\sigma^2/\epsilon^2)$ this lemma matches the exponential convergence of TV distance shown in~\citet{chen2022improved}.
% However, drawing samples from exact $p_{k+1|k+\frac{1}{2},b}(\vx^\prime|\vx, \vb)$ requires to use rejection sampling with impractical initialization, e.g., the stationary point of $f_{\vb}(\vx)$.
% Hence, we prefer to consider the error propagation when $\delta_k\not=0$. Specifically, we have
\begin{theorem}
    \label{thm:comp_conv_sps}
    Suppose Assumption~\ref{con_ass:lips_loss}-\ref{con_ass:var_bound} hold, and Alg.~\ref{alg:sps} satisfies:
    \begin{itemize}[leftmargin=*]
        \item We have $\eta_k\le \frac{1}{2L}$ for all $k\in\{0,1,\ldots, K-1\}$.
        \item The initial particle $\hat{\rvx}_0$ is drawn from the standard Gaussian distribution on $\R^d$.
        \item Line 5 is implemented by some specific inner sampler, achieving
            \begin{equation*}
                \KL{\hat{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)}{{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)} \le \delta_k
            \end{equation*}
        for all $k\in\{0,1,\ldots, K-1\}$.
    \end{itemize}
    Then, we have
    \begin{equation}
        \small
        \label{ineq:sps_tv_bound}
        \begin{aligned}
            \TVD{\hat{p}_{K}}{p_*} \le &\sqrt{\frac{1}{2}\sum_{i=0}^{K-1} \delta_i} +  \sigma \sqrt{\sum_{i=0}^{K-1} \frac{\eta_i}{2|\rvb_i|}} \\
            & + \sqrt{\frac{(1+L^2)d}{4\alpha_*}} \cdot \prod_{i=0}^{K-1} \left(1+\alpha_* \eta_i\right)^{-1}.
        \end{aligned}
    \end{equation}
\end{theorem}
%\dz{first summarize the error term, like how to understand different terms, how to adjust to make the sampling error small. then discuss the issue of \citet{altschuler2023faster},}
Theorem~\ref{thm:comp_conv_sps} provides the general upper bound of the TV distance between the underlying distribution of particles returned by Alg.~\ref{alg:sps} and the target distribution $p_*$. 
The first term in Eq~\ref{ineq:sps_tv_bound} represents the accumulated error of the inexact sampling from $p_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)$, i.e., Line 5 of Alg~\ref{alg:sps}.
The second term represents the approximation error using stochastic gradients, and the last term represents the error from deterministic proximal samplers.
To achieve an $\epsilon$-TV distance to the target distribution $p_*$, one may have to choose a small error tolerance of inexact sampling, i.e., $\delta_k=\epsilon^2$, to control the first term of Eq~\ref{ineq:sps_tv_bound}.
Besides, it still requires a large enough mini-batch size, i.e., $|\rvb_i|=\Theta(1/(\sigma \epsilon)^2)$ and the mixing time, i.e., $\sum_{i=0}^{K-1}\eta_i = \Theta(\log(1/\epsilon))$, to make the last two terms of Eq~\ref{ineq:sps_tv_bound} small, respectively.

Notably, the implementation of the proximal sampler in~\citet{altschuler2023faster} also allows inexact sampling from $p_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)$ in the second stage update, and requires the underlying distribution of returned particles, i.e., $\hat{p}_{k+1|k+\frac{1}{2},b}(\cdot|\vx,\vb)$ to satisfy Eq.~\ref{def:transition_kernel_norgo} with a small $\delta_k$.
However, they only consider the deterministic setting, i.e., $\vb=\{1,2,\ldots,n\}$, and requires initializing Line 5 of Alg.~\ref{alg:sps} with certain stationary points $\vx_*$ of $f$.
Hence, directly applying their analysis may require finding stationary points in each iteration, as the function $f_{\vb}$ changes, which may take substantially more time.
This is because, when $p_*$ only satisfies LSI, the function $f_{\vb}$ may not be convex.
Finding an $\epsilon$-approximate stationary point of a general non-convex function requires $\mathcal{O}(\epsilon^{-4})$~\cite{nesterov2013introductory} for stochastic gradient descent, which is unacceptable in sampling algorithms.
%Although~\citet{altschuler2023faster} also provides the analysis when Line 5 of Alg.~\ref{alg:sps} is initialized by arbitrary $\vz_0\in \R^d$, the gradient complexity will still depend on $\log\|\vz_0 - \vx_*\|$ to achieve Eq.~\ref{def:transition_kernel_norgo}.
Therefore, the implementation of~\citet{altschuler2023faster} still remains a concern without exact information, or even only with inexact information, about the stationary points of $f$. 
%\dz{mention the reference to eps4, the second part regarding using arbitrary z0 can be deleted.... looks super werid. we alreayd mention that they consider determinstic version, do not need to say more}

In our analysis, combining proper Langevin-based MCMC with a $\hat{\rvx}_{k+1/2}$ mean Gaussian-type initialization, the gradient complexity for achieving Eq.~\ref{def:transition_kernel_norgo} will only depend on $\log\|\hat{\rvx}_{k+1/2}\|^2$ rather than stationary points $\vx_*$, which will be explicitly shown in the next section. Considering the expected gradient complexity, it requires to characterize $\E_{\hat{p}_{k+1/2}}[\log\|\hat{\rvx}_{k+1/2}\|^2]$, which can be readily upper bounded by $\log[\E_{\hat{p}_{k+1/2}}[\|\hat{\rvx}_{k+1/2}\|^2]]$. This implies that we further need to control the second moment of the particles. This is conducted in the following lemma.
\begin{lemma}
    \label{lem:2ndmoment_bound}
    Suppose Assumption~\ref{con_ass:lips_loss}-\ref{con_ass:var_bound} hold, and the second moment of the underlying distribution of $\hat{\rvx}_{k}$ is $M_k$, then we have 
    \begin{equation*}
        M_{k+1} \le 24 M_k + 4\eta_k \delta_k +24\eta_k^2 \sigma^2/{|\rvb|}+ 28M  + 24\eta_k d.
    \end{equation*}
\end{lemma}

This bound may seem to be large as $M_k$ exhibit an exponential increasing rate. However, we remark that only $\log(M_k)$ will appear in our calculation of the gradient complexity rather than $M_k$ itself. Then, let $K$ be the number of total steps, which can be chose to be $\tilde{\mathcal{O}}(L/\alpha^*)$, then $M_K$ will be controlled by $\exp(K)$ and so that $\log(M_k)$ can be controlled by $K=\tilde{\mathcal{O}}(L/\alpha^*)$, which will not heavily affect the total gradient complexity.



% Although this upper bound increases exponentially, benefit from the unbiased Markov chain of proximal samplers, the iteration number of Alg.~\ref{alg:sps}, i.e., $K$ is $\tilde{O}(L/\alpha_*)$ with proper choice of $\eta_k$.
% Therefore, $\log M_{K}$ will only bring an additional $\tilde{O}(L/\alpha_*)$ factor and not dominate the total gradient complexity.



==> 0_contents/050experiments_icml_ver.tex <==
\section{Experiments}
\label{sec:exp}
In this section, we will first provide our experimental settings. 
Then, for a fair comparison with SGLD, we implement the proximal sampler with SPS-SGLD and show their sampling performance with different dimensions.
More experimental results are deferred to Appendix~\ref{sec:appendix_exp}.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
         \includegraphics[width=3.8cm]{0_figs/opt_dim_tv.pdf} &
         \includegraphics[width=3.8cm]{0_figs/10d_eta_tv.pdf}
    \end{tabular}
    \caption{\small The graph in the left column shows the TV distance estimation, i.e., $\mathrm{TV}(\hat{p}_K, p_*)$ when SGLD and SPS-SGLD chose their optimal hyper-parameters under different dimensions. The graph in the right column denotes the TV distance estimation when SGLD and SPS-SGLD chose different step sizes and $d=10$.}
    \label{fig:tv_diff}
    \vspace{-10pt}
\end{figure}

\noindent\textbf{Experimental Settings.} Here, we consider the component $e^{-f_i}$ shares a similar definition in~\citet{zou2019sampling}, i.e., $e^{-f_i(\vx)}\coloneqq e^{-{\left\|\vx - \vb - \vmu_i\right\|^2}/2} + e^{-{\left\|\vx - \vb + \vmu_i\right\|^2}/2}$,
where the number of input data $n=100$, the dimension $d\in\{10, 20, 30, 40, 50\}$, the bias vector $\vb = (3,3,\ldots, 3) \cdot $, and the data input $\sqrt{d/10}\cdot \vmu_i\sim \mathcal{N}(\overline{\vmu}, \mI_{d\times d})$ with $\overline{\vmu} = (2,2,\ldots, 2)$.
Here, we require the input data to shrink with the growth of $d$, which keeps the distances between different modes for each $e^{-f_i}$.
Since~\citet{zou2019sampling} had proven the function $f_i$ is dissipative, which implies the LSI property of $e^{-f_i}$ and $e^{-f}$, we omit the discussion about the property of $f_i$ in this section. 

For the common hyper-parameter settings of SGLD and SPS-SGLD, we fix the number of stochastic gradient oracles as $12000$ and the mini-batch size for each iteration as $1$.
We enumerate the step size of SGLD and the inner step size of SPS-SGLD from $0.2$ to $1.4$. 
Besides, the inner loops' iterations and the outer loops' step sizes are grid-searched with $[20, 40, 80]$ and $[1.0, 4.0,10.0]$.
Besides, we use the formulation $\mathrm{TV}(\hat{p}_K, p_*)\coloneqq \frac{1}{2d}\sum_{i=1}^d \mathrm{TV}(\hat{p}_{K,i}, p_{*,i})$
to estimate total variation distances between the target distribution and the underlying distribution of returned particles, where $\hat{p}_{K,i}$ and $p_{*,i}$ are the marginal distributions of the $i$-th coordinate.
For $1$d distributions, their densities can be approximated by the histogram of particles.

\noindent\textbf{Experimental Results.} We first show the optimal TV distance to the target distribution $p_*$ obtained by SGLD and SPS-SGLD under different dimensions in the left column of  Fig.~\ref{fig:tv_diff}.
Since we consider different problems when using different dimensions, the sampling error does not necessarily increase when $d$ increases.
It can be clearly observed that the optimal TV distance of SPS-SGLD is at least $0.5$ smaller than that of SGLD in all our dimension settings, which means SPS-SGLD presents a significantly better performance in this synthetic task.
Specifically, we investigate the changes in the TV distance with the growth of step sizes for both SPS-SGLD and SGLD, and show the results in the right column Fig.~\ref{fig:tv_diff}.
Although the absolute values of these two algorithms vary a lot, their changing trends are very similar.
When the step size is small, both SPS-SGLD and SGLD describe the local landscape of a single mode well. 
With the growth of step sizes, they can gradually cover all modes, whereas SPS-SGLD achieves a lower TV distance since it can cover modes and keep the local landscape well with a smaller step size.
Besides, we provide show distributions of particles' projections under different stochastic gradient oracles when $d=10$ and the optimal step sizes are chosen in Fig.~\ref{fig:illustration_exp}.
According to the contour of the projected negative log density of $p_*$, we note that SPS-SGLD can cover all modes with a more accurate variance estimation compared with SGLD.
It demonstrates that SPS-SGLD generates more reasonable samples with different stochastic gradient oracles from another perspective.


==> 0_contents/070impact.tex <==
\section*{Impact Statement}
This paper presents work whose goal is to advance the sampling field of Machine Learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.

==> 0_figs/sps_explain.tex <==
\usetikzlibrary{decorations.pathreplacing}

\usetikzlibrary{decorations.pathreplacing}

\begin{tikzpicture}

\node at (5,4.9) {The deterministic process};

\node at (5,-1) {The stochastic process};

\filldraw (0,4) circle (0.05); \node at (-0.2, 3.7) {\textcolor{red}{$\tilde{p}_{(1,1),0}$}}; 
\draw[-latex]  (0,4)--(0.5,4);
\draw[densely dotted] (0.5,4)--(1.5,4);
\draw[-latex]  (1.5,4)--(2,4);
\filldraw (2,4) circle (0.05); \node at (1.8, 3.7) {$\tilde{p}_{(k,1),0}$}; 
\filldraw (5,4) circle (0.05); \node at (4.8, 3.7) {$\tilde{p}_{(k,1),\eta}=\tilde{p}_{(k,2),0}$};
\draw[-] (2,4)--(5,4);
\draw[-] (5,4)--(8,4);
\filldraw (8,4) circle (0.05); \node at (7.8, 3.7) {$\tilde{p}_{(k,2),\eta}$}; 
\draw[-latex]  (8,4)--(8.5,4);
\draw[densely dotted] (8.5,4)--(9.5,4);
\draw[-latex]  (9.5,4)--(10,4);
\filldraw (10,4) circle (0.05); \node at (9.8, 3.7) {\textcolor{blue}{$\tilde{p}_{(K,2),\eta}\quad\approx$}}; 
\draw[dashed] (10,4)--(11, 4);
\filldraw (11,4) circle (0.05); \node at (11.2, 3.7) {$p_*$}; 

\filldraw (0,0) circle (0.05); \node at (-0.2, -0.3) {\textcolor{red}{$p_{(1,1),0}$}}; 
\draw[-latex]  (0,0)--(0.5,0);
\draw[densely dotted] (0.5,0)--(1.5,0);
\draw[-latex]  (1.5,0)--(2,0);
\filldraw (2,0) circle (0.05); \node at (1.8, -0.3) {$p_{(k,1),0}$}; 
\filldraw (5,0) circle (0.05); \node at (4.8, -0.3) {$p_{(k,1),\eta}=p_{(k,2),0}$}; 
\draw[-] (2,0)--(5,0);
\draw[-] (5,0)--(8,0);
\filldraw (8,0) circle (0.05); \node at (7.8, -0.3) {$p_{(k,2),\eta}$}; 
\draw[-latex]  (8,0)--(8.5,0);
\draw[densely dotted] (8.5,0)--(9.5,0);
\draw[-latex]  (9.5,0)--(10,0);
\filldraw (10,0) circle (0.05); \node at (9.8, -0.3) {\textcolor{blue}{$p^{(K,2)}_{\eta}$}}; 


\draw[dashed] (0,0)--(0,4);
\draw[dashed] (10,0)--(10,4);
\node [rotate=90] at (-0.3,2) {$=$};
\draw[-] (11,4)--(10,0);
\node [rotate=72] at (10.8,2) {$\approx$};

\filldraw (2,1) circle (0.05); \node at (1.8, 1.3) {$\vzero$}; 
\filldraw (8,1) circle (0.05); \node at (8.3, 1.3) {$\vzero$}; 
\filldraw (5,1) circle (0.05); \node at (5.3, 1.3) {$\grad\ln p_{(k,1),\eta}(,\vb)$}; 
\draw[-latex, dashed] (2,0)--(2,1);
\draw[-latex, dashed] (8,0)--(8,1);
\draw[-latex, dashed] (5,0)--(5,1);



\filldraw (2,3) circle (0.05); \node at (1.8, 2.7) {$\vzero$}; 
\filldraw (8,3) circle (0.05); \node at (8.3, 2.7) {$\vzero$}; 
\draw[-latex, dashed] (2,4)--(2,3);
\draw[-latex, dashed] (8,4)--(8,3);
\filldraw (5,3) circle (0.05); \node at (5.3, 2.7) {$\grad\ln \tilde{p}_{(k,1),\eta}$}; 
\draw[-latex, dashed] (5,4)--(5,3);


%\draw [decorate,decoration={brace,amplitude=10pt}, blue] (5,3) -- (8,3);
%\node at (6.4,3.5) {\textcolor{blue}{Term 2}};

%\draw [decorate,decoration={brace,amplitude=10pt}, red] (8,3) -- (8,1);
%\node at (8,2) {\textcolor{red}{Term 3}};

\end{tikzpicture}
